Haptic-Assisted Collaborative Robot Framework for Improved Situational Awareness in Skull Base Surgery

Skull base surgery is a demanding field in which surgeons operate in and around the skull while avoiding critical anatomical structures including nerves and vasculature. While image-guided surgical navigation is the prevailing standard, limitation still exists requiring personalized planning and recognizing the irreplaceable role of a skilled surgeon. This paper presents a collaboratively controlled robotic system tailored for assisted drilling in skull base surgery. Our central hypothesis posits that this collaborative system, enriched with haptic assistive modes to enforce virtual fixtures, holds the potential to significantly enhance surgical safety, streamline efficiency, and alleviate the physical demands on the surgeon. The paper describes the intricate system development work required to enable these virtual fixtures through haptic assistive modes. To validate our system's performance and effectiveness, we conducted initial feasibility experiments involving a medical student and two experienced surgeons. The experiment focused on drilling around critical structures following cortical mastoidectomy, utilizing dental stone phantom and cadaveric models. Our experimental results demonstrate that our proposed haptic feedback mechanism enhances the safety of drilling around critical structures compared to systems lacking haptic assistance. With the aid of our system, surgeons were able to safely skeletonize the critical structures without breaching any critical structure even under obstructed view of the surgical site.

==> Scrap/1_Introduction.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}

% \begin{enumerate}
    %\item What is Skull-base surgery, and what are the difficulties\\
    Skull-base surgery is a highly specialized and complex subset of neurosurgery and otolaryngology that focuses on the treatment of various surgical procedures at the base of the skull. Due to the intricate nature of the anatomical structures involved, ranging from critical blood vessels and nerves to vital brain components, the surgical procedure necessitates extreme precision and skill. One minor error can result in severe consequences, including nerve damage that could cause facial paralysis and other significant complications \cite{cousins_2008}.
    %\item Image-guided surgical navigation (IGSN), IGSN is useful with all the feedback//
    To address these challenges, Image-Guided Surgical Navigation (IGSN) has been introduced as an invaluable tool to improve surgical accuracy and enhance patient safety. IGSN systems mostly use preoperative scans of patient anatomy by Computed Tomography (CT) or Magnetic Resonance Imaging (MRI) images for surgical planning. [Add a few robotic systems for IGSN] These systems provide surgeons with real-time spatial information and a variety of feedback mechanisms, aiding them in navigating through the complex landscape of the surgical site. For example, [Add few feedback mechanisms]
    %\item Not many of them are actually tested in the real-surgery situation (In Skull base surgery)\\
    Despite the potential advantages of IGSN, it is crucial to note that most of these systems have yet to be rigorously tested in real-world surgical scenarios, particularly in the realm of skull-base surgery. No currently available surgical system is approved for use in the skull base. \cite{HEUERMANN20201077}. [Can add few examples for the current systems] This gap between technological advancements and their clinical application highlights the need for more exhaustive and comprehensive studies that may include cadavers to validate these technologies.
    %\item Introduce the previous works(FIVRS \cite{FIVRS2023} and SDF simulation paper \cite{ishida2023improving})\\
    One of our coauthors has implemented the fully immersive Virtual reality, FIVRS \cite{FIVRS2023}, which introduced a framework for Virtual Reality Simulation in skull-base surgery, and our group also facilitates similar simulator\cite{ishida2023improving} to test and compare the different modalities that use of Signed Distance Fields (SDF) for improving surgical surgical awareness. While both studies demonstrate the potential of technological integration into skull-base surgery, they primarily focus on simulations, leaving room for real-world validations.
    %\item Apply force feedback(Best modality from the SDF paper) and test the effectiveness using cadaver//
    The primary objective of this study is to bridge the gap between simulated surgical practices and real-world applications. Drawing from the most effective modality of force feedback as outlined in the paper \cite{ishida2023improving}, we aim to conduct a validation experiment on cadavers to assess the applicability, efficacy, and safety of our proposed IGSN in skull-base surgery.
% \end{enumerate}

%Add a nice figure that explains the system overview.
\begin{figure}[htp]%
\centering
\includegraphics[width=.45\textwidth]
% TODO: Change the size later
{Figures/Main_Figure_draft.jpeg}
\caption{Placeholder figure for first pitch}\label{fig:Main_Figure}
%\vspace{-5pt}
\end{figure}

Specify the main contribution of this paper:
\begin{enumerate}
    \item Demonstrating the proposed assistance method for skull base surgery, which is designed to protect the complicated-shaped anatomy such as facial nerve
    \item Rapid and comprehensive pipeline from preoperative CT to interoperative assistance 
    \item Clinical validation using cadavers and surgeons
    \item Open source and modular library for a wide range of surgical procedure
\end{enumerate}



==> Scrap/2_RelatedWork.tex <==
\section{Related Work}

% VF > Teleoperated vs Cooperative > Forbidden (x mm margin) and Guidance > Our work - Haptic guidance for skullbase 
% Category: Type of device (teleoperated vs cooperative robots), type of control system (impedance vs admittance) and the degree of automation (fully-automated vs. semi-autonomous control) Teleoperated vs Cooperative 
Multiple works~\cite{bowyer2013active}) have introduced robotic systems to assist human during manipulation tasks.
These works can be broadly categorized into the degree of automation (fully-automated vs. semi-autonomous control) they offer. 
For the sake of brevity, we will focus on robotic systems suitable for head and neck procedures.
%these procedures were designed . 
While there are some advantages to autonomously drill bone~\cite{dillon2016making}, autonomous surgery requires precise planning for every eventuality, and type of surgical approach, and does not benefit from the surgeon’s inherent procedural knowledge, technical skill and perceptual feedback.
In contrast, for cooperative system, both the surgeon and the robot holds the drill simultaneously, allowing drill motion proportional to the surgeon’s applied force surgeons while abiding by active constraints placed by the controller. 
The safety constraints can be activated when the the drill approaches a critical stricture and remains inactive otherwise.
In this work, we use a cooperatively controlled robot for robotic assisted drilling. 

Within the context of safety-driven assistance, 
% used by “warning” systems to enhance information available to the surgeon or robotic systems to enforce safety barriers around critical structures 
\begin{itemize}
    % Warning
    %\item \cite{cho2013warning} developed a warning navigation system when certain structures have been approached during drilling of temporal bone. 
    % Phantom - forbidden VF
    \item \cite{ding2021volumetric} performed phantom drilling experiment to show that planar virtual fixtures can be enforced by a cooperatively controlled robotic system. While these constraints are useful in defining the robotic workspace or operating range, they are not suitable for providing appropriate feedback in the vicinity of the critical structures. %These virtual fixtures are only able to restrict motion.
    \item \cite{lim2016semi,yoo2017cadaver} showed the utility of a cooperative robot for mastoidectomy procedures using cadaveric specimens. A safety shutoff margin of 3 mm is enforced between critical structures and the drill. Drill stops frequently. No comparison between with and without assistance
\end{itemize}


%Within the context of control system that implement active constraints, cooperative robots use admittance control and move when commanded by the 

Other VF papers - Robotic mastoidectomy \cite{danilchenko2011robotic}
% A majority of prior work applies virtual fixtures for teleoperation. THey can be designed to replace a portion of the surgical task. Perhaps
%In contrast to forbidden-region based virtual fixtures that keep the manipulator's tool within its task space and out of forbidden regions of the workspace, guidance based virtual fixtures (GVFs) assist the user in moving the robot manipulator along desired paths or surfaces in the workspace. \cite{abbott2007haptic,bowyer2013active}
% [Rephrase] In an admittance-type cooperative manipulation system, the robot motion is proportional to the user’s applied force, which is measured by a force sensor. To create GVFs, an instantaneous preferred direction is defined based on the position of the robot relative to the desired path or surface. The applied force is then decomposed into components in the preferred direction and in other, non-preferred directions. By eliminating the commanded motion due to the applied force in the non-preferred directions, we create a passive guidance along the preferred direction. \cite{bettini2004vision}

SDF papers

\begin{itemize}
    \item INF paper \cite{zhang2023Implicit} used implicit neural field (INF) to derive distance fields from patient volumetric imaging. (teleoperation, not evaluated on real surgery)
    
    Similar motivation and application. Takes too much time to train the INF. With access to high-enough resolution CT/MRI scans, using the signed distance field will provide similar results in less time. Some anatomy/surgery is time-sensitive and needs to start the surgery soon after the scans.

    \item recent papers that propose haptic assistance but no clinical use

    \item The work that is Too specific to the one medical procedure

\end{itemize}

Our paper focuses on providing haptic feedback to effectively guiding the drill motion away from critical structures, instead of enforcing hard safety barriers. 
